From RAG to RICHES: Retrieval Interlaced with Sequence Generation

We present RICHES, a novel approach that interleaves retrieval with sequence generation tasks. RICHES offers an alternative to conventional RAG systems by eliminating the need for separate retriever and generator. It retrieves documents by directly decoding their contents, constrained on the corpus. Unifying retrieval with generation allows us to adapt to diverse new tasks via prompting alone. RICHES can work with any Instruction-tuned model, without additional training. It provides attributed evidence, supports multi-hop retrievals and interleaves thoughts to plan on what to retrieve next, all within a single decoding pass of the LLM. We demonstrate the strong performance of RICHES across ODQA tasks including attributed and multi-hop QA.

==> prompts/blended_generation.tex <==
\begin{table*}[ht]
\begin{center}

\begin{tabular}{c|p{0.8\linewidth}|}
\toprule
\textit{C: Propositions} & << Apollo 17 was the last mission to the Moon. >> 
\newline
<< Apollo 17 landed on the Moon on December 11, 1972. >> \\
\midrule
\textit{C: Propositions, U: Ans} &  
<< Apollo 17 was the last mission to the Moon. >> 
\newline
<< Apollo 17 landed on the Moon on December 11, 1972. >>
\newline
answer: December 11, 1972 \\
\midrule
\textit{C: Prop. , U: Kw, Ans} & keyword: Apollo 17 
\newline 
<< Apollo 17 was the last mission to the Moon. >> 
\newline
keyword: Apollo 17 date << Apollo 17 landed on the Moon on December 11, 1972. >>
\newline
answer: December 11, 1972 \\
\bottomrule
\end{tabular}
\caption{Illustrative outputs for blended generation described in \Cref{sec:blended}}
\label{prompt:blended_output}
\end{center}
\end{table*}

==> tables/additional_baselines.tex <==
\begin{table*}[ht]
\begin{center}

\begin{tabular}{ll|cc}
\toprule
\multirow{2}{*}{Retriever} & \multirow{2}{*}{Answerer}  & \multicolumn{2}{c}{Hotpot} \\
& &  F1 & AutoAIS \\ 
\midrule
Decomp & Flan-T5-xxl  & 22.1 & - \\
\midrule
\multicolumn{4}{l}{\loci{}}
\llmm{}   & None  & 41.0 & 36.5 \\
\end{tabular}
\caption{Comparison of conventional Iterative retrieval methods \textit{Decomp} \citep{khot2022decomposed} with \loci{}}
\label{tab:additional_baseline}
\end{center}
\end{table*}


==> tables/num_prop.tex <==
\begin{table}[ht]
\begin{center}

\begin{tabular}{l|c}
\toprule
Dataset  &  Avg Propositions \\
\midrule
NQ & 1.6 \\
Hotpot &  2.5 \\
Musique &  2.8 \\
\bottomrule
\end{tabular}

\caption{Average propositions for each dataset with \llmm{}.}
\label{tab:num_prop}
\end{center}
\end{table}

==> tex/discussions.tex <==
\section{Discussions}


% \subsection{PT vs IT vs FT}
% Compare few-shot vs finetuned model performance. PT vs IT models.


% \subsection{Scale}
% Comparison between LLM-S, M, L.

% \subsection{Cost Analysis}
% Here’s a hand-wavy cost analysis:

% \paragraph{Dense Retrieval}

% Each search-unit is embedded into a vector. For sequence S, cost of embedding using model $M$ is $~O(|S|^2*|M|)$.

% Embedding the full corpus $~O(|C||S|^2*|M|)$.

% \paragraph{Constrained Generation}

% LLM inference is only incurred at query time, it is independent of corpus size.



